Patterns In The Coefficients Of Powers Of Polynomials Over A Finite Field

We examine the behavior of the coefficients of powers of polynomials over a finite field of prime order. Extending the work of Allouche-Berthe, 1997, we study a(n), the number of occurring strings of length n among coefficients of any power of a polynomial f reduced modulo a prime p. The sequence of line complexity a(n) is p-regular in the sense of Allouche-Shalit. For f=1+x and general p, we derive a recursion relation for a(n) then find a new formula for the generating function for a(n). We use the generating function to compute the asymptotics of a(n)/n^2 as n approaches infinity, which is an explicitly computable piecewise quadratic in x with n= [p^m/x] and x is a real number between 1/p and 1. Analyzing other cases, we form a conjecture about the generating function for general a(n). We examine the matrix B associated with f and p used to compute the count of a coefficient, which applies to the theory of linear cellular automata and fractals. For p=2 and polynomials of small degree we compute the largest positive eigenvalue, \lambda, of B, related to the fractal dimension d of the corresponding fractal by d= \log_2(\lambda). We find proofs and make a number of conjectures for some bounds on \lambda, and upper bounds on its degree.

==> biblio.tex <==
% This is biblio.tex
 
%% Enter your formatted bibliography information into this file.
%% Use a format appropriate to a journal in your field.

%% DO NOT TOUCH THIS LINE UNLESS YOU REALLY KNOW WHAT YOU'RE DOING
\begin{thebibliography}{99}

%% Enter your formatted \bibitem{key} info here.

\bibitem{Skye:norfolk} Stamey, Skye E.: Everything's Illegal
in Virginia! {\it Norfolk Daily News}, 12 July 1992: 11(C).

\bibitem{AmySz:cookbook} Szczepa\'nski, Amy F.: {\it 100
Meals Using Ingredients That Your Mother Thinks Are Weird}. 
San Diego: Bench Press, 1997.

\bibitem{Mikey:tresbouchet} Szczepa\'nski, Michael T.: Strange Things 
that I have Catapulted into our Neighbors' Yards. {\it Journal
of Home Use of Medieval Siege Weapons}. {\bf 271} (10 December 1991):
19-76.

%% YOU SHOULD NOT HAVE TO CHANGE THIS LINE
\end{thebibliography}

